Fast Similarity Sketching

We consider the $\textit{Similarity Sketching}$ problem: Given a universe $[u] = \{0,\ldots, u-1\}$ we want a random function $S$ mapping subsets $A\subseteq [u]$ into vectors $S(A)$ of size $t$, such that the Jaccard similarity $J(A,B) = |A\cap B|/|A\cup B|$ between sets $A$ and $B$ is preserved. More precisely, define $X_i = [S(A)[i] = S(B)[i]]$ and $X = \sum_{i\in [t]} X_i$. We want $E[X_i]=J(A,B)$, and we want $X$ to be strongly concentrated around $E[X] = t \cdot J(A,B)$ (i.e. Chernoff-style bounds). This is a fundamental problem which has found numerous applications in data mining, large-scale classification, computer vision, similarity search, etc. via the classic MinHash algorithm. The vectors $S(A)$ are also called $\textit{sketches}$. Strong concentration is critical, for often we want to sketch many sets $B_1,\ldots,B_n$ so that we later, for a query set $A$, can find (one of) the most similar $B_i$. It is then critical that no $B_i$ looks much more similar to $A$ due to errors in the sketch. The seminal $t\times\textit{MinHash}$ algorithm uses $t$ random hash functions $h_1,\ldots, h_t$, and stores $\left ( \min_{a\in A} h_1(A),\ldots, \min_{a\in A} h_t(A) \right )$ as the sketch of $A$. The main drawback of MinHash is, however, its $O(t\cdot |A|)$ running time, and finding a sketch with similar properties and faster running time has been the subject of several papers. (continued...)

==> LSH/speed-up.tex <==
\subsection{Speeding Up the Filtering using Word Parallelism}
Currently we are using $\Theta(1)$ time per matching in the filtering step, but
we will show how to use amortized $O\left( \frac{\log w}{w} \right)$ time per
matching. Thus by setting
$K = \ceil{\frac{\log\left( \frac{n \log w}{w} \right)}{2\log(1/j_2)}}$
and $L = 6\ceil{(1/j_1)^K}$ we will get an algorithm that uses
$O\left( n \left(\frac{n \log w}{w}\right)^\rho \log(1/\eps) + \sum_{A \in \calF} \abs{A} \right)$
space and $O\left( \left(\frac{n \log w}{w}\right)^\rho \log(1/\eps) + \abs{Q}\right)$ query time.
To get this improved filtering time, the crucial idea is to work
on several of the $O(L^2)$ matches in parallel. We can then use the following result which will
be proved in \Cref{sec:word_parallelism} using techniques somewhat similar to those in
\cite{DBLP:journals/jal/Thorup02}.
\begin{lemma}\label{lem:word_parallelism}
    Given $m$ words, $t_0, \ldots, t_{m - 1}$, of length $w$ which are each split up
    into $k = \floor{\frac{w}{d}}$ bit segments, 
    $k_0^{(0)}, \ldots, k_0^{(k - 1)}, \ldots, k_{m - 1}^{(0)}, \ldots, k_{m - 1}^{(k - 1)}$,
    of size $d$, that is, each of the bit segments consists of $d$ bits. Then
    there exists an algorithm, which does not use multiplication, that in $O(m + \log d)$
    time produces new words,
    $t_0, \ldots, t_{m - 1}$, such that, the bit segment $t_i^{(j)}$ interpreted
    as an integer is the number of 1-bits in $k_i^{(j)}$ for every $i \in [m]$ and
    $j \in [k]$.
\end{lemma}
Now it should be noted that filtering scheme described below only uses Chernoff-type
bounds on the similarity, hence the filtering scheme can be used to improve
the space and time of any LSH data structure.

We are now going to describe how we can improve the filtering using \Cref{lem:word_parallelism}.
Note that with $K = \ceil{\frac{\log\left( \frac{n \log w}{w} \right)}{2\log(1/j_2)}}$ we
expect $O\left(\frac{w}{\log w} L^2\right)$ bad matches in each of the good experiments.
We define 
\[
    J_{Q}(A^{*}) = \setbuilder{i \in [M]}
        {\left( \calM_{Q}(A^{*})[i] > 0 \right) 
        \wedge
        \left( \sum_{A \in \calF_{bad}(Q)} \calM_{Q}(A)[i] \le C \frac{w}{\log w} L^2 \right)
    }
\]
where $\calM_{Q}(A)[i]$ is the number of matches of $A \in \calF$ in the $i$'th
experiment where $i \in [M]$.
The same arguments as in \Cref{app:filtering} give 
that $\abs{J_{Q}(A^{*})} = \Theta(\log(1/\eps))$ with probability
at least $1 - \frac{\eps}{4}$. Now we split the experiments into two groups:
The experiments that have less than
$2C \frac{w}{\log w} L^2$ matches and the experiments that have more than
$2C \frac{w}{\log w} L^2$. If an experiments has many matches then we just pick
a random match.

Now we have to explain what we do with the experiments with few matches. During
creation of the data structure we will create a sketch $P(A)$ of size
$l = \Theta\left(\max(\log(n), \log(1/\eps))\right)$ using the minwise 1-bit hashing trick
for each element $A \in \calF$. Then for each experiment $i \in [M]$ we will
sample $d$ coordinates, $l^{(i)}_0, \ldots, l^{(i)}_{d - 1}$, uniformly at random,
and save the small sketch $P_i(A) = (P(A)[l^{(i)}_0], \ldots, P(A)[l^{(i)}_{d - 1}])$
for each $A \in \calF$, where $d = O(\log w)$. Note that we can pack these sketches
into $O(\log w)$ bits, and hence we can pack $O\left(\frac{w}{\log w} \right)$
sketches into one word.

By using a union bound and Chernoff bounds we get that there exists constants
$c_1$ and $c_2$ such that $c_1 \frac{1 + j_1}{2} - c_2 \frac{1 + j_2'}{2}$ is
positive and constant, and for each $A \in \calF_{bad}$
$
    \frac{\sum_{i \in [l]} [P(A)[i] = P(Q)[i]]}{l} \le c_2 \frac{1 + j_2'}{2}
$
and for each $A \in \calF_{good}$ then
$
    \frac{\sum_{i \in [l]} [P(A)[i] = P(Q)[i]]}{l} \ge c_1 \frac{1 + j_1}{2}
$
with probability at least $1 - \frac{\eps}{4}$.

Choosing the threshold $\gamma = \frac{c_1 \frac{1 + j_1}{2} - c_2 \frac{1 + j_2'}{2}}{2}$ we
get that
\begin{align*}
    \Prp{\sum_{j \in [d]} [P_i(A)[j] = P_i(Q)[j]] \ge \gamma d} \le e^{\Omega(d)} = w^{-2}
\end{align*}
for $A \in \calF_{bad}$, and
\begin{align*}
    \Prp{\sum_{j \in [d]} [P_i(A)[j] = P_i(Q)[j]] \le \gamma d} \le e^{\Omega(d)} = w^{-2}
\end{align*}
for $A \in \calF_{good}$ for every experiment $i \in [M]$. Now we say that a match
survives the filtering if $\sum_{j \in [d]} [P_i(A)[j] = P_i(Q)[j]] \le \gamma d$,
and that word survives the filtering step if contains a match that survives
the filtering.

If a word consists of $\frac{w}{d}$ bad matches
then the probability that any of the matches survives the filtering is at most
$w^{-1}$. So we expect that at most $O(L^2/w)$ words consisting of all bad matches
survive the filtering step.

Using \Cref{lem:word_parallelism} we can check $L^2$ words whether they survive
the filtering in
$O(L + \lg d) = O\left( \left( \frac{n \log w}{w} \right)^\rho \right)$ time.

Now we want to use our previous filtering scheme. We choose a suitable
constant $C_2 = O(1)$. If less than $C_2 L^2 / w$
words survives the filtering step then less than $C_2 L^2$ matches survives the
filtering step so using the previous filtering scheme takes $O(L^2)$ time. If
more than $C_2 L^2 / w$ words survives the filtering step then less than a
constant fraction of them consists of only bad matches. If we pick a random
word then with constant probability it contains
a match, $A$, with $J(A, Q) > j_2$. This step takes $O(L^2/w)$ time
which give us the result.

